GHOST: Building blocks for high performance sparse linear algebra on heterogeneous systems

While many of the architectural details of future exascale-class high performance computer systems are still a matter of intense research, there appears to be a general consensus that they will be strongly heterogeneous, featuring "standard" as well as "accelerated" resources. Today, such resources are available as multicore processors, graphics processing units (GPUs), and other accelerators such as the Intel Xeon Phi. Any software infrastructure that claims usefulness for such environments must be able to meet their inherent challenges: massive multi-level parallelism, topology, asynchronicity, and abstraction. The "General, Hybrid, and Optimized Sparse Toolkit" (GHOST) is a collection of building blocks that targets algorithms dealing with sparse matrix representations on current and future large-scale systems. It implements the "MPI+X" paradigm, has a pure C interface, and provides hybrid-parallel numerical kernels, intelligent resource management, and truly heterogeneous parallelism for multicore CPUs, Nvidia GPUs, and the Intel Xeon Phi. We describe the details of its design with respect to the challenges posed by modern heterogeneous supercomputers and recent algorithmic developments. Implementation details which are indispensable for achieving high efficiency are pointed out and their necessity is justified by performance measurements or predictions based on performance models. The library code and several applications are available as open source. We also provide instructions on how to make use of GHOST in existing software packages, together with a case study which demonstrates the applicability and performance of GHOST as a component within a larger software stack.

==> ghost_building_blocks.tex <==
\begin{SCtable}
    \centering
    \begin{tabular}{llll}
        \hline
        \textbf{Function} & \textbf{CPU} & \textbf{GPU} & \textbf{PHI} \\
        \hline
        \hline
        axpy & H & H & H \\ 
        axpby & H & H & H \\ 
        scal & H & H & H \\ 
        dot & H & H & H \\ 
        vaxpy & H & H & H \\ 
        vaxpby & H & H & H \\ 
        vscal & H & H & H \\ 
        aug\_spmmv & G$_\text{I,H}$(H) & G$_\text{H}$(H) & G$_\text{I,H}$(H) \\
        gemm & L & L & L \\
        tsmttsm & G$_\text{I,H}$(L) & L & G$^\text{I}$ \\
        tsmttsm\_kahan & G$_\text{I,H}(\times)$ & $\times$ &
        G$_\text{H}(\times)$ \\
        tsmm & G$_\text{I,H}$(L) & L & G$_\text{H}$ \\
        tsmm\_inplace & G$_\text{H}$(L$^\dagger$) & L$^\dagger$ & G$_\text{H}$(L$^\dagger$) \\
        \hline
    \end{tabular}
    \caption{Currently available numerical kernels in \ghost. Note that all BLAS
        level 1/2 functions are block vector-enabled.\\
        ``H'': High-level implementation. \\
        ``L'': A library is called. \\
        ``G'': The kernel is auto-generated at compile time (cf.
        \cref{sec:implementation}), fallback version
        in parentheses. \\
        $^\dagger$: In-/output vector gets cloned. \\
        $\times$: Non-Kahan version gets called along with a warning. \\
        $\cdot_\text{H}$: Auto-generated high-level code. \\
        $\cdot_\text{I}$: Auto-generated intrinsics code.
    }
    \label{tab:math_kernels}
\end{SCtable}
\Cref{tab:math_kernels} gives an overview of currently existing numerical kernels in
\ghost\ and details about their implementation. This list is likely to be extended in
future development\new{, especially once \ghost\ gains broader attention from other
communities}.



